Concatenation of Markov processes

We investigate the concatenation of Markov processes. Our primary concern is to utilize processes constructed in this manner for Monte Carlo integration. To enable this using conventional methods, it is essential to demonstrate the Markov property and invariance with respect to a given target distribution. We provide mild sufficient conditions for this. Our main result is the identification of the generator of the concatenation of Markov processes. This result provides the theoretical foundation for Monte Carlo methods based on this construction.

==> nomenclature.tex <==
\setlength{\nomlabelwidth}{4cm}

\renewcommand\nomgroup[1]{%
    \item[\bfseries
    \ifstrequal{#1}{A}{Analysis}{%
    \ifstrequal{#1}{F}{Functional Analysis}{%
    \ifstrequal{#1}{M}{Measure Theory}{%
    \ifstrequal{#1}{P}{Probability Theory}{%
    \ifstrequal{#1}{T}{Topology}{}}}}}%
]}

% analysis
\nomenclature[A]{$\left\|\;\cdot\;\right\|_\infty$}{Supremum norm}
\nomenclature[A]{$\operatorname{id}_\probabilityspace$}{Identity map on $\probabilityspace$}

% measure theory
\nomenclature[M]{$\mathcal M_1(\measurablespace,\measurablesystem)$}{Set of probability measures on $(\measurablespace,\measurablesystem)$ (p. \pageref{inline:probability-measures})}
\nomenclature[M]{$\mathcal M_{\le1}(\measurablespace,\measurablesystem)$}{Set of sub-probability measures on $(\measurablespace,\measurablesystem)$ (p. \pageref{inline:sub-probability-measures})}



==> text/a_topology.tex <==
\section{}

\begin{proposition}[measurability invariance under $\sigma$-algebra extension]\label{prop:measurability-invariance}
    
\end{proposition}



Let $(\probabilityspace,\eventsystem)$ be a measurable space.

\begin{lemma}[generator of join]\label{lem:generator-of-join}
    % \bigbreak\noindent Let $\filtration_i\subseteq\eventsystem$ be $\cap$-stable with $\probabilityspace\in\filtration_1\cap\filtration_2$ $\Rightarrow$ \begin{enumerate}[(i)]
    %     \item \begin{equation}
    %         \generatorsystem:=\left\{\filtrationset1\cap \filtrationset2:\filtrationseti\in\filtration_i\right\}
    %     \end{equation} is $\cap$-stable with $\probabilityspace\in\generatorsystem$.
    %     \item \begin{equation}
    %         \sigma(\generatorsystem)=\filtration_1\vee\filtration_2.
    %     \end{equation}
    % \end{enumerate}
    % \begin{proof}[Proof\textup:\nopunct]
    %     \leavevmode
    %     \begin{enumerate}[(i)]
    %         \item Let $\generatorseti\in\generatorsystem$ $\Rightarrow$ $\exists\left(\filtrationset^{(i)}_1,\filtrationset^{(i)}_2\right)\in\filtration_1\times\filtration_2$ with \begin{equation}
    %             \generatorseti=\filtrationset^{(i)}_1\cap\filtrationset^{(i)}_2
    %         \end{equation} and hence (since $\filtration_i$ is $\cap$-stable) \begin{equation}
    %             \generatorset1\cap \generatorset2=\left(\filtrationset^{(1)}_1\cap \filtrationset^{(1)}_2\right)\cap\left(\filtrationset^{(2)}_1\cap \filtrationset^{(2)}_2\right)\in\generatorsystem.
    %         \end{equation}
    %         \item \leavevmode\begin{itemize}[$\circ$]
    %             \item $\probabilityspace\in\filtration_1\cap\filtration_2$ $\Rightarrow$ \begin{equation}
    %                 \filtration_1\cup\filtration_2\subseteq\generatorsystem.
    %             \end{equation}
    %             \item \begin{listclaim}\label{lem:generator-of-join-claim1}
    %                 \begin{equation}
    %                     \generatorsystem\subseteq\filtration_1\vee\filtration_2.
    %                 \end{equation}
    %                 \begin{proof}[Proof\textup:\nopunct]
    %                     \leavevmode
    %                     \begin{itemize}[$\sq$]
    %                         \item Let $\generatorset\in\generatorsystem$ $\Rightarrow$ $\exists \filtrationseti\in\filtration_i$ with \begin{equation}
    %                             \generatorset=\filtrationset1\cap \filtrationset2.
    %                         \end{equation}
    %                         \item $\filtrationseti\in\filtration_1\cup\filtration_2\subseteq\filtration_1\vee\filtration_2$ and $\filtration_1\vee\filtration_2$ is $\cap$-stable $\Rightarrow$ \begin{equation}
    %                             \generatorset\in\filtration_1\vee\filtration_2.
    %                         \end{equation}
    %                     \end{itemize}
    %                 \end{proof}
    %             \end{listclaim}
    %             \item \autoref{lem:generator-of-join-claim1} $\Rightarrow$ Claim.
    %         \end{itemize}
    %     \end{enumerate}
    % \end{proof}
\end{lemma}


==> text/concatenation_of_processes.tex <==
\section{Concatenation of processes}\label{sec:concatenation-of-processes}

Let \begin{itemize}[$\circ$]
    \item $\indexset:=[1,n]\cap\mathbb N$ for some $n\in\mathbb N\uplus\{\infty\}$;
    \item $(\probabilityspace_\indexsetelement,\eventsystem_\indexsetelement)$ be a measurable space and \begin{equation}
        \begin{split}
             \probabilityspace&:=\bigtimes_{\indexsetelement\in\indexset}\probabilityspace_\indexsetelement;\\
             \eventsystem&:=\bigvee_{\indexsetelement\in\indexset}\eventsystem_\indexsetelement;
        \end{split}
    \end{equation}
    \item $\left(\filtration^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$ be a filtration on $(\probabilityspace_i,\eventsystem_\indexsetelement)$ and \begin{equation}
        \begin{split}
            \tilde{\filtration}^{(\ge\indexsetelement)}_\timepoint&:=\filtration^{(\indexsetelement)}_\timepoint\times\bigtimes_{\substack{\secondindexsetelement\in\indexset\\\secondindexsetelement>\indexsetelement}}\probabilityspace_\secondindexsetelement;\\\tilde{\filtration}^{(\indexsetelement)}_\timepoint&:=\bigtimes_{\secondindexsetelement=1}^{\indexsetelement-1}\probabilityspace_\secondindexsetelement\times\tilde{\filtration}^{(\ge\indexsetelement)}_\timepoint
        \end{split}
    \end{equation} for $\timepoint\ge0$;
    \item $\lifetime_\indexsetelement:\probabilityspace_\indexsetelement\to[0,\infty)$ be $\eventsystem_\indexsetelement$-measurable.
\end{itemize}

\begin{remark}
    \begin{equation}
        \secondfiltration^{(\indexsetelement)}_\timepoint:=\sigma\left(\bigcup_{\prevtimepoint\in[0,\;\timepoint]}\left\{\lifetime_\indexsetelement\le\timepoint\right\}\right)\;\;\;\text{for }\timepoint\ge0
    \end{equation} is the smallest filtration on $(\probabilityspace_\indexsetelement,\eventsystem_\indexsetelement)$ with respect to which $\lifetime_\indexsetelement$ is a stopping time. Let \begin{equation}
        \thirdfiltration^{(\indexsetelement)}_\timepoint:=\filtration^{(\indexsetelement)}_\timepoint\vee\secondfiltration^{(\indexsetelement)}_\timepoint
    \end{equation} and \begin{equation}
        \begin{split}
            \tilde\thirdfiltration^{(\ge\indexsetelement)}_\timepoint&:=\thirdfiltration^{(\indexsetelement)}_\timepoint\times\bigtimes_{\substack{\secondindexsetelement\in\indexset\\\secondindexsetelement>\indexsetelement}}\probabilityspace_\secondindexsetelement;\\\tilde\thirdfiltration^{(\indexsetelement)}_\timepoint&:=\bigtimes_{\secondindexsetelement=1}^{\indexsetelement-1}\probabilityspace_\secondindexsetelement\times\tilde{\thirdfiltration}^{(\ge\indexsetelement)}_\timepoint
        \end{split}
    \end{equation} for $\timepoint\ge0$.
    \begin{flushright}
        $\square$
    \end{flushright}
\end{remark}

Let \begin{equation}
    \lifetimesum_\secondindexsetelement(\outcome):=\sum_{\indexsetelement=1}^\secondindexsetelement\lifetime_\indexsetelement(\outcome_\indexsetelement)\;\;\;\text{for }\outcome\in\bigtimes_{\indexsetelement=1}^\secondindexsetelement\probabilityspace_\indexsetelement.
\end{equation}

Let $\probabilityprojection_\indexsetelement$ denote the projection from $\probabilityspace$ onto the $\indexsetelement$th coordinate.

Let \begin{equation}
    \tilde\lifetime_\indexsetelement:=\lifetime_\indexsetelement\circ\probabilityprojection_\indexsetelement
\end{equation} and \begin{equation}
    \tilde\lifetimesum_\secondindexsetelement:=\sum_{\indexsetelement=1}^\secondindexsetelement\tilde\lifetime_\indexsetelement.
\end{equation}

To simplify the subsequent definition, we write\footnote{We slightly abuse notation to simplify the definition and the subsequent usage of it. If $\indexsetelement=1$, then \begin{equation}
    \event_{(\outcome_1,\:\ldots\:,\:\outcome_{\indexsetelement-1})}=\event.
\end{equation}} \begin{equation}
    \event_{(\outcome_1,\:\ldots\:,\:\outcome_{\indexsetelement-1})}:=\left\{\left(\outcome_j\right)_{\substack{\secondindexsetelement\in\indexset\\\secondindexsetelement\ge\indexsetelement}}\in\bigtimes_{\substack{\secondindexsetelement\in\indexset\\\secondindexsetelement\ge\indexsetelement}}\probabilityspace_\secondindexsetelement:(\outcome_\secondindexsetelement)_{\secondindexsetelement\in\indexset}\in\event\right\}
\end{equation} for $\event\subseteq\probabilityspace$ and $(\outcome_1,\ldots,\outcome_{\indexsetelement-1})\in\bigtimes_{\secondindexsetelement=1}^{\indexsetelement-1}\probabilityspace_\secondindexsetelement$.

\begin{lemma}\label{lem:filtration-induced-by-concatenation}
    \begin{equation}
        \thirdfiltration_\timepoint:=\left\{\event\in\eventsystem\;\middle|\;\begin{aligned}&\left(\event\cap\left\{\timepoint<\tilde\lifetimesum_i\right\}\right)_{(\outcome_1,\:\ldots\:,\:\outcome_{\indexsetelement-1})}\in\tilde{\thirdfiltration}^{(\ge\indexsetelement)}_{\timepoint-\lifetimesum_{\indexsetelement-1}(\outcome_1,\:\ldots\:,\:\outcome_{\indexsetelement-1})}\\&\text{for all }\outcome\in\{\lifetimesum_{\indexsetelement-1}\le\timepoint\}\text{ and }\indexsetelement\in\indexset\end{aligned}\right\}\;\;\;\text{for }\timepoint\ge0
    \end{equation} is a filtration on $(\probabilityspace,\eventsystem)$.
    \begin{proof}[Proof\textup:\nopunct]
    \end{proof}
\end{lemma}

Let \begin{itemize}[$\circ$]
    \item $(\measurablespace_\indexsetelement,\measurablesystem_\indexsetelement)$ be a measurable space and \begin{equation}
        \begin{split}
            \measurablespace&:=\bigcup_{\indexsetelement\in\indexsetelement}\measurablespace_\indexsetelement;\\\measurablesystem&:=\bigvee_{\indexsetelement\in\indexset}\measurablesystem_\indexsetelement;
        \end{split}
    \end{equation}
    \item $\left(\localprocess^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$ be an $(\measurablespace_\indexsetelement,\measurablesystem_\indexsetelement)$-valued $\left(\filtration^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$-adapted process on $(\probabilityspace_\indexsetelement,\eventsystem_\indexsetelement)$ and \begin{equation}
        \tilde\localprocess^{(\indexsetelement)}:=\localprocess^{(\indexsetelement)}\circ\probabilityprojection_\indexsetelement.
    \end{equation}
\end{itemize}

\begin{lemma}
    Let $\indexsetelement\in\indexset$ $\Rightarrow$ \begin{equation}
        \left.\tilde\localprocess^{(\indexsetelement)}\right|_{\probabilityspace\times[0,\;\timepoint]}^{-1}(\measurablesystem)=\bigtimes_{\secondindexsetelement=1}^{\indexsetelement-1}\probabilityspace_\secondindexsetelement\times\left.\localprocess^{(\indexsetelement)}\right|_{\probabilityspace\times[0,\;\timepoint]}^{-1}(\measurablesystem_\indexsetelement)\times\bigtimes_{\substack{\secondindexsetelement\in\indexset\\\secondindexsetelement>\indexsetelement}}\probabilityspace_\secondindexsetelement\;\;\;\text{for all }\timepoint\ge0.
    \end{equation} In particular, if $\left(\localprocess^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$ is $\left(\filtration^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$-adaptive/progressive, then $\left(\tilde\localprocess^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$ is $\left(\tilde\filtration^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$-adaptive/progressive.
    \begin{proof}[Proof\textup:\nopunct]
    \end{proof}
\end{lemma}

Let $\deadstate\not\in\measurablespace$ and $(\measurablespace^\ast,\measurablesystem^\ast)$ denote the one-point extension of $(\measurablespace,\measurablesystem)$.

\begin{proposition}
    If $\left(\localprocess^{(1)}_\timepoint\right)_{\timepoint\ge0}$ is $\left(\filtration^{(1)}_\timepoint\right)_{\timepoint\ge0}$-adaptive and $\left(\localprocess^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$ is $\left(\filtration^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$-progressive for all $\indexsetelement\in\indexset$ with $\indexsetelement\ge2$, then \begin{equation}
        \concatenatedprocess_\timepoint:=\left.\begin{cases}
            \tilde\localprocess^{(\indexsetelement)}_{\timepoint-\tilde\lifetimesum_{\indexsetelement-1}}&\text{, if }\indexsetelement\in\indexset\text{ and }\timepoint\in\left[\tilde\lifetimesum_{\indexsetelement-1},\tilde\lifetimesum_\indexsetelement\right);\\
            \deadstate&\text{, otherwise}
        \end{cases}\right\}\;\;\;\text{for }\timepoint\ge0
    \end{equation} is an $(\measurablespace^\ast,\measurablesystem^\ast)$-valued $(\thirdfiltration_\timepoint)_{\timepoint\ge0}$-adapted process on $(\probabilityspace,\eventsystem)$.
    \begin{proof}[Proof\textup:\nopunct]
    \end{proof}
\end{proposition}


\section{Concatenation of Markov processes}

Let $\left(\localsemigroup^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$ be a Markov semigroup on $(\measurablespace_\indexsetelement,\measurablesystem_\indexsetelement)$. Assume $\left(\left(\localprocess^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0},\left(\probabilitymeasure^{(\indexsetelement)}_\point\right)_{\point\in\measurablespace_\indexsetelement}\right)$ is a realization of $\left(\localsemigroup^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}$ on $\left(\probabilityspace_\indexsetelement,\eventsystem_\indexsetelement,\left(\filtration^{(\indexsetelement)}_\timepoint\right)_{\timepoint\ge0}\right)$.


